CAMOUFLAGE: Exploiting Misinformation Detection Systems Through LLM-driven Adversarial Claim Transformation

Automated evidence-based misinformation detection systems, which evaluate the veracity of short claims against evidence, lack comprehensive analysis of their adversarial vulnerabilities. Existing black-box text-based adversarial attacks are ill-suited for evidence-based misinformation detection systems, as these attacks primarily focus on token-level substitutions involving gradient or logit-based optimization strategies, which are incapable of fooling the multi-component nature of these detection systems. These systems incorporate both retrieval and claim-evidence comparison modules, which requires attacks to break the retrieval of evidence and/or the comparison module so that it draws incorrect inferences. We present CAMOUFLAGE, an iterative, LLM-driven approach that employs a two-agent system, a Prompt Optimization Agent and an Attacker Agent, to create adversarial claim rewritings that manipulate evidence retrieval and mislead claim-evidence comparison, effectively bypassing the system without altering the meaning of the claim. The Attacker Agent produces semantically equivalent rewrites that attempt to mislead detectors, while the Prompt Optimization Agent analyzes failed attack attempts and refines the prompt of the Attacker to guide subsequent rewrites. This enables larger structural and stylistic transformations of the text rather than token-level substitutions, adapting the magnitude of changes based on previous outcomes. Unlike existing approaches, CAMOUFLAGE optimizes its attack solely based on binary model decisions to guide its rewriting process, eliminating the need for classifier logits or extensive querying. We evaluate CAMOUFLAGE on four systems, including two recent academic systems and two real-world APIs, with an average attack success rate of 46.92\% while preserving textual coherence and semantic equivalence to the original claims.

==> sections/4_problem_statement.tex <==
% This work investigates black-box attacks against evidence-based misinformation detection systems, where attackers have no access to the system's internal architecture, parameters, or confidence scores, and can only observe binary decisions for input claims. A claim $x$ is a short text span (typically 1-2 sentences) that makes a specific assertion that can be verified against evidence. Let $f(x) \in \{0,1\}$ represent a black-box misinformation detection system that evaluates claims against evidence to output a binary decision, where $1$ denotes true claims and $0$ denotes false claims. Let $y^*$ be the ground truth label for claim $x$.

% An adversarial rewriting $\tilde{x}$ of the original claim $x$ aims to cause the classifier's prediction to differ from the ground truth label, formally expressed as $f(\tilde{x}) \neq y^*$. The adversarial rewriting must satisfy two key constraints: (1) semantic equivalence and (2) linguistic coherence. For semantic equivalence, we require that $\tilde{x}$ maintains semantic equivalence to $x$ according to an appropriate similarity function $S(\tilde{x}, x) \geq \tau_S$, where $\tau_S$ is a predefined threshold. Additionally, we require that a semantic equivalence function $\mathrm{Sem}(\tilde{x}, x) = 1$ confirms that the core assertion remains unchanged. For linguistic coherence, we require that $\mathrm{Coh}(\tilde{x}) = 1$, ensuring the rewritten text maintains grammatical correctness and readability.
